CHAPTER: Exploiting Convolutional Neural Network Adapters for Self-supervised Speech Models

Self-supervised learning (SSL) is a powerful technique for learning representations from unlabeled data. Transformer based models such as HuBERT, which consist a feature extractor and transformer layers, are leading the field in the speech domain. SSL models are fine-tuned on a wide range of downstream tasks, which involves re-training the majority of the model for each task. Previous studies have introduced applying adapters, which are small lightweight modules commonly used in Natural Language Processing (NLP) to adapt pre-trained models to new tasks. However, such efficient tuning techniques only provide adaptation at the transformer layer, but failed to perform adaptation at the feature extractor. In this paper, we propose CHAPTER, an efficient tuning method specifically designed for SSL speech model, by applying CNN adapters at the feature extractor. Using this method, we can only fine-tune fewer than 5% of parameters per task compared to fully fine-tuning and achieve better and more stable performance. We empirically found that adding CNN adapters to the feature extractor can help the adaptation on emotion and speaker tasks. For instance, the accuracy of SID is improved from 87.71 to 91.56, and the accuracy of ER is improved by 5%.

==> 2.RelatedWork.tex <==
%\section{Related Works}
%\label{sec:related}
%\vspace{-5pt}

%\subsection{Adapter Approach} 
%wav2vec ASR
%focus on the difference on this work and previous adapter on speech work
%In the field of speech processing tasks, adapters have also been utilized for efficient SSL tuning. Using adapters on Wav2vec2 for efficient tuning for ASR has been proposed~\cite{thomas2022efficient}. \cite{hou2021exploiting} proposed SimAdapter for explicitly learning knowledge from adapters. More recently, \cite{chen2022exploring} proposed a unified framework for adapters applications to a wide range of speech processing tasks. The above works utilized transformer adapters on speech processing tasks, gaining promising results; however, they did not designed an adapter approach specifically for SSL speech models, which contains a CNN-based feature extractor and transformer layers. 
%In our work, in addition to applying adapters on transformer layers, we also applied residual adapter to adapt more global information, which might benefit for speaker and emotion related tasks.

%\subsection{The SUPERB benchmark}
%SUPERB~\cite{yang2021superb} is a framework to benchmark SSL models on 10 speech tasks by learning task-specific predictions heads on top of the frozen shared SSL models. In the SUPERB benchmark, the authors freezed the upstream SSL model, and learned the downstream model according to the downstream task. To investigate the effectiveness of our proposed SpeechAdapter, we conduct our experiment on the SUPERB benchmark,based on the parameter-efficient framework proposed by \cite{chen2022exploring}.

%As more powerful SSL models are being proposed with more promising performance on various tasks, researchers continually try to find extensive evaluation methods to assess model performance, in the hope of understanding the capability of the learned representation in these models. 

==> Figures/basic_residual_block.tex <==
\begin{figure}[h]
%\vspace{-20pt}
      \centering
      \includegraphics[width=0.45\textwidth]{Figures/ConvBlock.png}
      \caption{
        Illustration of the residual adapter in the feature extractor.
      }
\label{fg:overview}
\end{figure}



==> Table/cross_validation_er.tex <==
\begin{table}[]
\centering
%\vspace*{-15pt}
\begin{tabular}{c|c}

\hline
Output channel                             & ER             \\ 
\hline
finetune    &63.94\\
512                           & 65.44          \\

256                                            & 65.16          \\

128                                          & 65.75          \\

64                                           & 64.58          \\
 \hline 

\end{tabular}

\caption{cross validation with CNN adapter layer shrinking}
\label{tab:cross validation on er}
\end{table}
